Online non-convex optimization with imperfect feedback

We consider the problem of online learning with non-convex losses. In terms of feedback, we assume that the learner observes - or otherwise constructs - an inexact model for the loss function encountered at each stage, and we propose a mixed-strategy learning policy based on dual averaging. In this general context, we derive a series of tight regret minimization guarantees, both for the learner's static (external) regret, as well as the regret incurred against the best dynamic policy in hindsight. Subsequently, we apply this general template to the case where the learner only has access to the actual loss incurred at each stage of the process. This is achieved by means of a kernel-based estimator which generates an inexact model for each round's loss function using only the learner's realized losses as input.

==> App-Test.tex <==
%----------------------------------------------------------------------
%%% APP: TEST
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is a sample appendix.

==> Conclusion.tex <==
%----------------------------------------------------------------------
%%% CONCLUSION
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is the conclusions section.

==> Impact.tex <==
%----------------------------------------------------------------------
%%% IMPACT
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is a theoretical work which does not present any foreseeable societal consequence.

==> Numerics.tex <==
%----------------------------------------------------------------------
%%% NUMERICS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is the numerics section.

==> fig/slice.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.194607843137255,0.453431372549019,0.632843137254902}
\definecolor{color1}{rgb}{0.881862745098039,0.505392156862745,0.173039215686275}
\definecolor{color2}{rgb}{0.229411764705882,0.570588235294118,0.229411764705882}
\definecolor{color3}{rgb}{0.75343137254902,0.238725490196078,0.241666666666667}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Slice\_at\_20000},
x grid style={white!69.0196078431373!black},
xlabel={data},
xmin=0.0013917371247088, xmax=1.00356562862972,
xmode=log,
xtick style={color=black},
xtick={0.0001,0.001,0.01,0.1,1,10,100},
xticklabels={\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\),\(\displaystyle {10^{2}}\)},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ylabel={Algo},
ymin=-0.5, ymax=3.5,
ytick style={color=black},
ytick={0,1,2,3},
yticklabels={GridAnytime\_g1.0\_nbarm10,GridAnytime\_g1.0\_nbarm100,KernelApproxAnytime\_g1.0\_grate0.67\_nbdiscr10000\_initw1.00\_wrate0.25\_e0e1.00\_eeR0.25,KernelApproxAnytime\_g1.0\_grate0.75\_nbdiscr10000\_initw1.00\_wrate0.25\_e0e1.00\_eeR0.25}
]
\path [draw=white!23.921568627451!black, fill=color0, semithick]
(axis cs:0.186756467895622,-0.4)
--(axis cs:0.186756467895622,0.4)
--(axis cs:0.406424311300441,0.4)
--(axis cs:0.406424311300441,-0.4)
--(axis cs:0.186756467895622,-0.4)
--cycle;
\path [draw=white!23.921568627451!black, fill=color1, semithick]
(axis cs:0.18241668117044,0.6)
--(axis cs:0.18241668117044,1.4)
--(axis cs:0.46104393213428,1.4)
--(axis cs:0.46104393213428,0.6)
--(axis cs:0.18241668117044,0.6)
--cycle;
\path [draw=white!23.921568627451!black, fill=color2, semithick]
(axis cs:0.10165237048054,1.6)
--(axis cs:0.10165237048054,2.4)
--(axis cs:0.111758551976564,2.4)
--(axis cs:0.111758551976564,1.6)
--(axis cs:0.10165237048054,1.6)
--cycle;
\path [draw=white!23.921568627451!black, fill=color3, semithick]
(axis cs:0.165053747205085,2.6)
--(axis cs:0.165053747205085,3.4)
--(axis cs:0.174372558969514,3.4)
--(axis cs:0.174372558969514,2.6)
--(axis cs:0.165053747205085,2.6)
--cycle;
\addplot [semithick, white!23.921568627451!black]
table {%
0.186756467895622 0
0.0140261539630563 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.406424311300441 0
0.439993490842338 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0140261539630563 -0.2
0.0140261539630563 0.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.439993490842338 -0.2
0.439993490842338 0.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.00413115717854698 0
0.0067764335479345 0
0.0084433044048109 0
0.445916484429177 0
0.441555852012429 0
0.563171676518075 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.18241668117044 1
0.0505793823431512 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.46104393213428 1
0.649460530958295 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0505793823431512 0.8
0.0505793823431512 1.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.649460530958295 0.8
0.649460530958295 1.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.00297091683777634 1
0.0295332564501202 1
0.00187700652968029 1
0.737468561608841 1
0.693426386185231 1
0.744110113822354 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.10165237048054 2
0.0975846682186988 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.111758551976564 2
0.11662190355138 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0975846682186988 1.8
0.0975846682186988 2.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.11662190355138 1.8
0.11662190355138 2.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.0897350664511988 2
0.095186359882772 2
0.0935140123666294 2
0.117708672787127 2
0.116778953131257 2
0.118661664119505 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.165053747205085 3
0.159939581221649 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.174372558969514 3
0.177611654003803 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.159939581221649 2.8
0.159939581221649 3.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.177611654003803 2.8
0.177611654003803 3.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.155067067843934 3
0.158940866363285 3
0.155786506938132 3
0.1796011532512 3
0.178688028759334 3
0.17998797502049 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.276359249662769 -0.4
0.276359249662769 0.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.339444923279543 0.6
0.339444923279543 1.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.106770911461747 1.6
0.106770911461747 2.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.1697805940176 2.6
0.1697805940176 3.4
};

\nextgroupplot[
log basis x={10},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={Slice\_at\_199999},
x grid style={white!69.0196078431373!black},
xmin=0.000898539599028788, xmax=1.02661389398693,
xmode=log,
xtick style={color=black},
xtick={1e-05,0.0001,0.001,0.01,0.1,1,10,100},
xticklabels={\(\displaystyle {10^{-5}}\),\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\),\(\displaystyle {10^{2}}\)},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ylabel={Algo},
ymin=-0.5, ymax=3.5,
ytick style={color=black},
yticklabels={}
]
\path [draw=white!23.921568627451!black, fill=color0, semithick]
(axis cs:0.18582571375599,-0.4)
--(axis cs:0.18582571375599,0.4)
--(axis cs:0.408171181588031,0.4)
--(axis cs:0.408171181588031,-0.4)
--(axis cs:0.18582571375599,-0.4)
--cycle;
\path [draw=white!23.921568627451!black, fill=color1, semithick]
(axis cs:0.150641255024913,0.6)
--(axis cs:0.150641255024913,1.4)
--(axis cs:0.444843675347144,1.4)
--(axis cs:0.444843675347144,0.6)
--(axis cs:0.150641255024913,0.6)
--cycle;
\path [draw=white!23.921568627451!black, fill=color2, semithick]
(axis cs:0.0432465389996422,1.6)
--(axis cs:0.0432465389996422,2.4)
--(axis cs:0.0457892661501533,2.4)
--(axis cs:0.0457892661501533,1.6)
--(axis cs:0.0432465389996422,1.6)
--cycle;
\path [draw=white!23.921568627451!black, fill=color3, semithick]
(axis cs:0.0802249592663358,2.6)
--(axis cs:0.0802249592663358,3.4)
--(axis cs:0.0823787588215285,3.4)
--(axis cs:0.0823787588215285,2.6)
--(axis cs:0.0802249592663358,2.6)
--cycle;
\addplot [semithick, white!23.921568627451!black]
table {%
0.18582571375599 0
0.00254370632742183 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.408171181588031 0
0.44707768913241 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.00254370632742183 -0.2
0.00254370632742183 0.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.44707768913241 -0.2
0.44707768913241 0.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.00155411264228315 0
0.0018186654104751 0
0.00198536833214648 0
0.447670044762065 0
0.447233940092518 0
0.681043008093045 0
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.150641255024913 1
0.0501884467354861 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.444843675347144 1
0.548410797793242 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0501884467354861 0.8
0.0501884467354861 1.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.548410797793242 0.8
0.548410797793242 1.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.00123746039587669 1
0.00409456390021254 1
0.00132867616200423 1
0.745440613480706 1
0.549291751339879 1
0.714461517146559 1
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0432465389996422 2
0.0417593645454599 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0457892661501533 2
0.0464550881407363 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0417593645454599 1.8
0.0417593645454599 2.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0464550881407363 1.8
0.0464550881407363 2.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.0412281422335777 2
0.0416556187904412 2
0.0416553029964265 2
0.0475318984663824 2
0.0468464857047912 2
0.0466021738017056 2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0802249592663358 3
0.0785405555385311 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0823787588215285 3
0.0836627748539459 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0785405555385311 2.8
0.0785405555385311 3.2
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0836627748539459 2.8
0.0836627748539459 3.2
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=white!23.921568627451!black}, only marks]
table {%
0.0783404692283629 3
0.0783434619813121 3
0.07818058276584 3
0.0851674854640725 3
0.0837362812243631 3
0.0843728519417438 3
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.260911453243001 -0.4
0.260911453243001 0.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.327300739773854 0.6
0.327300739773854 1.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0445737419381306 1.6
0.0445737419381306 2.4
};
\addplot [semithick, white!23.921568627451!black]
table {%
0.0814079143381348 2.6
0.0814079143381348 3.4
};
\end{groupplot}

\end{tikzpicture}

